Revisiting Unnaturalness for Automated Program Repair in the Era of Large Language Models

Language models have improved by orders of magnitude with the recent emergence of Transformer-based Large Language Models (LLMs). LLMs have demonstrated their ability to generate natural code that is highly similar to code written by professional developers. One intermediate value an LLM can emit is entropy, which measures the naturalness of a token of code. We hypothesize that entropy can be used to improve the performance of Automated Program Repair (APR) tasks. While much progress has been made in Automated Program Repair (APR), fault localization techniques suffer from a lack of diversity in ranking scores, patch generation tools tend to be inefficient as all tests need to run before determining if a patch is likely to be correct, and patch ranking often suffers from the test-suite over-fitting problem. However, using an LLM directly for APR introduces concerns for training data leakage. In this work, we introduce a novel way of using the entropy of LLMs in combination with prior APR tools to improve all stages of APR. We show that entropy is highly complementary with prior fault localization tools. Our proposed re-ranking method achieves a 50% Top-5 score improvement over SBFL. We propose a patch-naturalness measurement, entropy-delta, to improve the efficiency of template-based repair techniques by ranking plausible patches before undergoing testing. When using entropy-delta for patch ranking and classification, our proposed method can rank correct patches more effectively than state-of-the-art machine learning tools with an 49% improvement in Top-1. Our work suggests that LLMs can be an effective addition to compliment prior APR tasks while minimizing both the test-suite overfitting problem and the LLM data leakage problem.

==> Makefile <==
DOC = main.tex

OTHERSOURCES := $(filter-out $DOC, $(wildcard sections/*.tex))
PDFLATEX = pdflatex -synctex=1 --shell-escape
BIBTEX = bibtex
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
TARDIR = $(DOC:.tex=-src)

.PHONY: pdf clean

pdf: $(DOC:.tex=.pdf)

all: pdf

%.pdf: %.tex $(OTHERSOURCES)
	${PDFLATEX} $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(PDFLATEX) $<; $(PDFLATEX) $<) ; true

clean:
	@\rm -f \
        $(DOC:.tex=.aux) \
        $(DOC:.tex=.log) \
        $(DOC:.tex=.out) \
        $(DOC:.tex=.dvi) \
        $(DOC:.tex=.pdf) \
        $(DOC:.tex=.ps)  \
        $(DOC:.tex=.bbl) \
        $(DOC:.tex=.blg) \
				$(DOC:.tex=-src.tar.gz)

veryclean: clean
	@\rm -r -f *~ *.log *.pdf *.gnuplot *.fdb_latexmk *.fls *.upa *.upb auto *.gz

tar: pdf
	@test -d $(TARDIR) || mkdir $(TARDIR)
	@cp Makefile *.{tex,bib,bst,cls} $(TARDIR)
	@tar cz $(TARDIR) > $(TARDIR).tar.gz
	@rm -rf $(TARDIR)


==> dead-text.tex <==


From introduction:

\iffalse 
As large language models of source code (Codex, CodeGen, inCoder) have been
scaled-up and improved, they are increasingly optimized to produce more
\textit{natural}, i.e., human-like code. These models have been explored in all
types of software engineering use cases, from nlp-code translation, type
inference, code search, all the way up to guided pair-programming. For such
tasks, partial correctness, or the semblance of readability may be valid
metrics. For automatic program repair, however, LLMs force us to contend with an
inherent misalignment: more natural generations are not necessarily any more
correct in the context of a program. 

In fact, their naturalness is often deceptive. A generated patch can look almost
identical to the reference patch, but upon testing, introduce an even more
pervasive bug. Explainability and reliability, two of LLM for code's biggest
weaknesses, are crucial in this domain. For repair in particular, the lack of
explainability in model-based fault localization and/or patch generation is
likely to seed mistrust among developers, who would replace their own complex
fault-localization reasoning with an estimate from a black-box. With respect to
reliability, even with the ability to generate patches cheaply, the cost of
iteratively testing and verifying their correctness remains. Running a
test-suite to verify a series of patches is not only time consuming, it is also
potentially misleading, as even a test-passing patch may break un-tested
functionality, or lead to unexpected behaviors over the lifespan of the project. 

The use of LLMs in APR is certainly not hopeless, however, confidence remains
especially crucial in this domain. Prior to the prevalence of LLMs, researchers
studied \textit{unnaturalness}---or how surprising a model finds some code---
~\todo{cite} as a means of distinguishing between buggy-and non-buggy code.
Here, we revisit unnaturalness in the era of large language models as repair
heuristic. We explore how entropy functions
\fi 

\iffalse
During training, LLMs minimize loss over a corpus of code. As models are exposed
to larger data sets, they are increasingly able to generate natural, i.e.,
probable code. From the opposite perspective, this means that their internal
probability counts are also stronger signals of unnatural, or improbable code.
Ray et al. theorized that unnaturalness may be correlated with bugginess, and
found evidence to that end with n-gram models~\cite{NAT} In the era of large
language models, recent work ~\cite{LLM-PATCH} has shown that larger models are
both better at patching programs and differentiating between buggy and non-buggy
statements. 

Despite the seeming promise of LLMs for software engineering, these models are
not trained with any awareness of the logical constructs that govern a program’s
execution. As such, their extension to the domain of APR requires careful
consideration. Alien code, for instance, which passes all tests but looks
extremely unnatural~\cite{CRIT}, would be suspected buggy by an entropy-based
repair technique. In the opposite case, if a bug is highly probable at a certain
point in a program, the model may simply re-generate the original bug, which it
(correctly) considers to be likely in that context. 

Given the usefulness, yet, inherent limitations, of unnaturalness in repair, we
propose a new method for integrating entropy (or unnaturalness) into APR. This
metric, which we term entropy delta, uses the difference in entropy between an
original statement and a proposed replacement to perform fault-localization and
suggest patches in the same process. 

\todo{describe the method}

For a given line and its surrounding context, if the model is able to generate a
patch that significantly reduces entropy, this means it has found a more
``natural" replacement. If, however, the patches do not significantly reduce
entropy, this means the model could not make the line more natural. We
hypothesize that buggy lines are more likely to fall into the first category,
and non-buggy lines, the second. 

A line may have high entropy because it is buggy, but is also may have entropy
simply due to a complex program structure. The advantage of comparing the
entropy of the original line with its proposed replacement (as opposed to just
measuring original entropy) is that the delta helps distinguishes between
possible causes of high entropy. In cases where both a line and its replacements
raw entropy are high, the entropy delta will be small, implying the original
line could not be improved due to program structure. In cases where a line's raw
entropy is high, but a replacement entropy is low, the entropy delta will be
large, implying the original line could be improved and is thus, potentially
buggy. 

We then explore a) how well entropy deltas work as a standalone repair method b)
whether or not they can improve existing program analysis-based repair
techniques. 

We answer the following research questions:

\begin{itemize}
    \item \textbf{RQ1} How effective is fault-localization with entropy-deltas
    at detecting bugs?
    \item \textbf{RQ2} How plausible are the patches generated during
    fault-localization?
    \item \textbf{RQ3} Can entropy distinguish between correct and incorrect
    patches that are both test-passing?
\end{itemize}

\fi

The typical Automatic program repair (APR) pipeline consists in three major
steps: fault-localization, patch generation, and patch validation. A variety of
methods ranging from purely analytical to purely statistical have been used for
each of these sub-tasks~\todo{cite}. In general, the analytical techniques have
the benefit of being sound, at the cost of being slow, whereas statistical
approaches have the benefit of increasing efficiency, at the cost of ignoring
program structure~\todo{cite}. The existence of this trade-off has limited the
effectiveness of APR. 

To bridge the gap, some researchers have attempted to encode program structure
in language models of code. These ``best of both worlds" solutions train along
with CFGs, ASTs, DFGs, type annotations, or other metadata that is removed by
tokenizers in generic LLMs. While more theoretically sound, the resulting models
tend to be limited by language and task specificity, require expensive
data-collection, pre-processing, and/or fine-tuning phases, and still may not
provide correctness guarantees.

Rather than discarding analysis altogether, an alternate approach is to try and
make it less expensive. In this formulation, a pre-trained LLM is queried as a
heuristic on top of analysis, rather than in place of it. The advantage of this
approach is that it requires no special training, making it a light-weight
addition to extant repair pipelines. By synthesizing techniques in this way, we
make use of the strengths of LLMs without discarding the useful ~\sk{looking for
a better word here, something more implying soundness or robustness} information
provided by program analysis.  

One of many possible methods for integrating LLMs into the repair pipeline is
entropy. Entropy can be understood as the inverse of probability, and generally
captures how "surprising" the model finds a given portion of code. Prior work
has shown both that entropy tends to be correlated with bugginess, and that
correct patches tend to lower entropy~\cite{NAT}~\cite{LLM-PATCH}. Taking these
two findings together, we hypothesize that the difference in entropy before and
after a change is made to code, or an entropy-delta, may be a stronger signal of
bugginess than entropy alone. To test our hypothesis, we evaluate the
effectiveness of using entropy-deltas for fault localization and patch
generation, comparing to entropy and program analysis alone, as well as in
combination ~\sk{pls help with phrasing}. Using entropy-deltas, we first perform
fault localization and patch generation in the same process. We then study
entropy-deltas as a heuristic through each phase of the repair pipeline. 

Our goal in doing so is not to propose a new repair technique, but rather, to
explore whether or not entropy calculations can be meaningfully combined with
traditional program analysis approaches to APR. For each stage of repair, we
formulate a series of experiments for evaluating this claim. For
fault-localization and patch generation, we collect a data set of 100 1-line
bugs from the defects4j benchmark. We then measure the propensity for
spectrum-based fault localization, entropy, and entropy-deltas, to correctly
localize the bug, both alone, and when used together. We find that
entropy-deltas substantially improve the ranking of buggy lines, by breaking
ties within equally suspicious chunks of code. Using each of the described FL
methods (as well as perfect FL as a baseline), we then record the number of
test-passing patches generated by the model given a limited number of repair
attempts. We find that, while test-passing patches almost always lower entropy,
many test-failing patches also lower entropy. For patch validation, we use a
data set provided and labeled by ~\todo{cite}, with one correct and many
test-passing but incorrect patches to a different set of defects4j bugs, which
are not restricted to a single line. We find that entropy-deltas identify the
correct patch on the first try for 75\% of the bugs.  

Our contributions are: 
\begin{itemize}
    \item  First Contribution
    \item  Second Contribution
    \item  Third Contribution
\end{itemize}


\textbf{1979: \cite{SOC}} DeMillo et al. argue that, like the process of
accepting a mathematical proof, the process of obtaining confidence in a
program's correctness is \textit{social}. The mere logical correctness of a
proof is irrelevant if experts cannot digest and comprehend it. Likewise, for
software engineers, having a system which takes in a program and returns,
"VERIFIED" or "NOT VERIFIED", means little to the programmer who cannot make
sense of how and why the system reached this conclusion. We apply a similar
argument to program repair, claiming that returning an incomprehensible patch,
and declaring the program "FIXED" or "NOT FIXED" is equally unhelpful. In
general, our approach prioritizes explainability and developer interaction over
fully automated techniques. 

~\textbf{2006: ~\cite{PATCH}} Weimer et al. make a similar argument, with
respect to early fault localization techniques. Their critique consists in two
main points. First, that, the utility of a bug finding tool lies not in how many
bugs it ~\textit{finds}, but in how many bugs it causes to be ~\textit{fixed}.
This informs their second assertion, that extant bug-finding tools, which
reported bugs in long, difficult to interpret, annotated back-traces were not
useful for real repair, as they caused developers to spent more time
understanding the error than actually fixing it. Their proposed solution was to
expose the bug by providing plausible patches. In showing an example patch, the
source of the error is exposed implicitly (rather than, explicitly through a
stack-trace). This made understanding bug reports easier, reducing the time and
cost of producing a fix. 


~\textbf{2013: ~\cite{AUTO}} Kim et al. present another APR technique called
PAR, in response to GenProg. Where GenProg uses random mutation techniques to
alter identified suspicious lines, PAR uses patterns learned over a dataset of
real patches. This method of patch generation was designed to produce more
human-readable code than the previously mentioned mutation strategy. Their
evaluation, which consisted in surveying people as to which patch
~\textit{appeared} more acceptable, found that a marginally larger number of
patches generated via this method were labeled as readable. Although future work
~\cite{CRIT} was highly critical of this evaluation strategy, PAR is relevant
for its early engagement with the concept of readability in machine generated
code. 

~\textbf{2014 ~\cite{CRIT}} Monperrus writes a critique of Kim et al.'s
paper~\cite{AUTO}. His primary issue surrounds defect classes, which scopes the
range of faults handled, and how they are handled by a given APR technique. This
is particularly relevant wrt evaluation criteria: without explicitly stating the
range of defect classes covered in their dataset, or how well PAR does across
each of them, PAR cannot be meaningfully compared with other techniques (i.e.
Genprog), which may just so happen to cover a different defect class. 

More broadly, Monperrus is arguing that ignoring the defect class sets the field
back, by obscuring the types of problems APR techniques are/are not succeeding
at. The second major thrust of the paper is regarding the misdirection of the
original problem (make the tests pass) to the problem solved by Kim et al. (make
the tests pass, and make the patches readable). He argues that the readability
of patches may or may not be relevant, depending on whether or not the system in
question is designed to do fully automated repair or to be a recommender system.
Again, by not clearly defining the problem domain, nor releasing the data set,
PAR cannot be compared to similar methods on equal footing. Ultimately, he
argues, this makes APR as a field fragmented and confused about its own
progression.

\sk{the "human readability" of the code may or may not be relevant. It is highly relevant in recommender systems, where the human must read/understand the patch. It is of low relevance in fully-automated approaches, where the patch is produced at execution time to prevent a crash, and can be later discarded. The question brings up the perceived/desired longevity of patches. Is this patch a temporary and desperate "fix", that can be further "fixed" later? Or, is it supposed to be naturally integrated into the human workflow, where Alien-ness is frowned upon?}

In other words, a patch that passes 100\% of the first test-suite is unlikely to
also pass 100\% of the second test-suite, demonstrating that the  ``correctness"
of the resulting patch is highly subject to the choice of test-cases in G\&V
(generate and validate) based repair.


~\textbf{2022 ~\cite{TRUST}} Noller et al. survey developers extensively about
their trust in automatically generated patches. They find that 72\% of
participants are willing to review auto-generated patches. 72\% are willing to
review up to 5 patches. 63\% would not wait longer than an hour. 72\% would not
wait longer than 30 minutes, and conclude that the ideal scenario is 5 or fewer
patches to review that can be generated in 30 minutes or less. They also find
that full developer trust requires a manual patch review. The root cause of the
bug is noted to be less desirable than the patch itself. Some participants
favored a list of potential patches. 93\% think passing additional test-cases
(as proposed by ~\cite{CURE}) are helpful for increasing trust. 

~\textbf{2022 ~\cite{PRACTICAL}} Large, pre-trained language models can yield
improvements, particularly with respect to the naturalness of patches and the
speed at which they are generated, relative to traditional program repair
techniques. 

Afzal et al.~\cite{TURING} distinguish between two types of patches: those
designed to produce a functional fix, but not necessarily to be read and
maintained (opaque), and those designed to be integrated into the development
process (transparent). For opaque fixes, as argued by ~\cite{CRIT}, there is no
need to avoid "alien" code, since the patches are time-sensitive, safety
critical, or designed to be changed later on by humans. For transparent patches,
however, there is a high importance place on the human-readability of patches,
as they are expected to exist long-term in a dynamic code environment. 



Introduction We posit that a higher entropy leads to the model finding a
sequence of code tokens less ``natural''. Recent advances in LLMs for code
mostly focus on patch generation~\cite{Infill_repair,Interfix,Prompt_repair},
but little work uses the perplexity of LLMs for all stages of APR. In this
paper, we explicitly revisit the potential role of naturalness in APR. We
evaluate entropy across three stages of automated program repair (APR): fault
localization, patch generation, and patch disambiguation. At a high level, APR
approaches begin by localizing a defect to be repaired to a smaller set of
program constructs, typically with ranking or suspiciousness scores (i.e., fault
localization). Such a technique then constructs one or more candidate repairs
(i.e., patch generation), at one or more candidate repair locations, before
evaluating them by running the modified program on the test cases (i.e., patch
validation). Some then perform additional analyses to filter, identify, or rank
patches that are correct according to users' intent, not just test-passing
(i.e., patch disambiguation). 

Meanwhile, recent trends in ML-informed patch generation~\cite{long_ml_patch,
patch_learning} use learned models to generate replacement code. However, recent
work on plausible patch ranking depend on information retrieved from the passed
tests, and little work has been done on improving patch ranking \textit{before}
tests have been deployed on a patch. Prior techniques typically use an
exhaustive patch search guided by available tests (i.e., generate patches until
a patch passes all tests)~\cite{TBar, patch-sim}. Liu et al.~\cite{efficiency}
perform an empirical evaluation on the efficiency of recent patch generation
techniques, and found that current template-based repair systems are highly
inefficient as they tend to generate a large percentage of irrelevant (test
failing) patch candidates. An average patch generation using the template-based
approach TBar~\cite{TBar} spends about 2\% of its total time forming a template,
6\% generating the patch, and 92\% on running tests on the generated patch. 


\aidan{I removed the variance numbers because they are not comparable across techniques, but added ties instead. I think only SBFL is good for motivation, the transfer one isn't needed}
For example, the variance on all suspicious scores assigned by
SBFL~\cite{abreu2006evaluation} is 0.038, and the variance on all suspicious
scores assigned by TransferFL~\cite{TransferFL} is 0.015 on the dataset \defj.

Entropy from LLMs offer clear potential advantages in each stage of the APR
domain. Language model based techniques are good at recognizing code that aligns
with human intuition, and often outperform heuristic or symbolic approaches when
it comes to replicating the ``readability'' of the human developer-produced
patch in the studied bug datasets~\cite{NAT} without the dependency on tests. We
posture that this advantage can apply to detecting incorrect and correct code,
both from the perspective of source code (for fault localization), non-plausible
patches (for patch generation efficiency), and plausible patches (for plausible
patch ranking). As a preliminary study, we find that the variance on all entropy
scores across lines of code in \defj is 0.071 (87\% higher than that of SBFL
suspicious scores). We hypothesize that the additional ``naturalness'' of
entropy scores can be used to improve the performance of both fault and patch
ranking, and the reduction of test time can be used to improve the efficiency of
all stages of APR.

In this work, we revisit unnaturalness based bug detection with entropy from
state-of-the-art LLMs, and introduce a novel use of entropy for patch
``naturalness''. We use entropy to measure patch quality, which we call the
entropy-delta, and score lines of code using both their prefix and suffix
context (i.e., computing entropy with a context window before and after the
line). We demonstrate across three evaluations that entropy judgements from
these models are highly valuable for fault localization, repair, and repair
efficiency. 


Prior work on the stages of APR suffer from a dependency of tests, assigning
similar scores to buggy and non-buggy lines, and an inefficient patch generation
process. Fault localization techniques employ test-coverage based
analysis~\cite{abreu2006evaluation}, graph neural network (GNN) for fault line
classification~\cite{DeepFL, TransferFL}, and finally large language model (LLM)
based fault localization~\cite{Llmao}. 
